Fully Automated Functional Fuzzing of Android Apps for Detecting Non-crashing Logic Bugs

Android apps are GUI-based event-driven software and have become ubiquitous in recent years. Obviously, functional correctness is critical for an app's success. However, in addition to crash bugs, non-crashing functional bugs (in short as "non-crashing bugs" in this work) like inadvertent function failures, silent user data lost and incorrect display information are prevalent, even in popular, well-tested apps. These non-crashing functional bugs are usually caused by program logic errors and manifest themselves on the graphic user interfaces (GUIs). In practice, such bugs pose significant challenges in effectively detecting them because (1) current practices heavily rely on expensive, small-scale manual validation (the lack of automation); and (2) modern fully automated testing has been limited to crash bugs (the lack of test oracles). This paper fills this gap by introducing independent view fuzzing, a novel, fully automated approach for detecting non-crashing functional bugs in Android apps. Inspired by metamorphic testing, our key insight is to leverage the commonly-held independent view property of Android apps to manufacture property-preserving mutant tests from a set of seed tests that validate certain app properties. The mutated tests help exercise the tested apps under additional, adverse conditions. Any property violations indicate likely functional bugs for further manual confirmation. We have realized our approach as an automated, end-to-end functional fuzzing tool, Genie. Given an app, (1) Genie automatically detects non-crashing bugs without requiring human-provided tests and oracles (thus fully automated); and (2) the detected non-crashing bugs are diverse (thus general and not limited to specific functional properties), which set Genie apart from prior work.

==> backup.tex <==
\begin{table*}[t]
	\footnotesize
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	%% increase table row spacing, adjust to taste
	\renewcommand{\arraystretch}{1}
	% if using array.sty, it might be a good idea to tweak the value of
	% \extrarowheight as needed to properly center the text within the cells
	
	\caption{App subjects used in our evaluation. \#L. \#Br., \#M., \#Cl. represent the numbers of code lines, branches, methods and classes, respectively.}
	\vspace*{-0.5pc}
	\label{table:app_subjects}
	\centering
	%% Some packages, such as MDW tools, offer better commands for making tables
	%% than the plain LaTeX2e tabular which is used here.
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|c|c|c|}
			\hline
			App Name &Feature Description &\tabincell{c}{Version} &\tabincell{c}{First\\Release} &\tabincell{c}{\#Google Play\\Installations} &\tabincell{c}{\#GitHub\\Stars} &\tabincell{c}{\#L.} &\tabincell{c}{\#Br.} & \tabincell{c}{\#M.}  & \tabincell{c}{\#Cl.} \\
			\hline \hline
			\emph{ActivityDiary} &Personal Diary & 1.4.0 &Oct. 2017 & 1K$\sim$5K &56 &4,238 &1,169 & 611 & 157 \\
			\emph{Transistor} &\tabincell{c}{Radio Program\\ Player}  & 3.2.2 &Oct. 2015 & 10K$\sim$50K & 254  &3,024 & 1,003 & 551 & 137 \\
			\emph{Tasks} &\tabincell{c}{Task Manager\\ \& Reminder} & 6.6.5 &Dec. 2008 &100K$\sim$500K &1.3K &31,757 & 8,386 & 6,187 & 984 \\
			\emph{UnitConverter} &Unit Converter & 5.5.1 &Jun. 2014 &1M$\sim$5M &144 &1,525 & 304 & 300 & 88 \\
			\emph{RadioDroid} &\tabincell{c}{Radio \\Streaming Player} & 0.79 &Jan. 2013 &50K$\sim$100K &323 &8,085 & 2,397 & 1,426 & 309 \\
			\emph{SkyTube} &\tabincell{c}{YouTube \\Video Player} & 2.97 &Nov. 2015 &100K$\sim$500K &843 &8,469 & 2,531 & 1,889 & 318 \\
			\emph{SimpleTask} &\tabincell{c}{Cloudless \\To-do Lists} & 10.3.0 &Mar. 2013 &10K$\sim$50K & 390 & 2,512 & 1,022 & 403 & 83 \\
			\emph{Fosdem} &\tabincell{c}{Conference \\Scheduler Browser} & 1.6.2 &Dec. 2013 &10K$\sim$50K & 111 & 5,563 & 1,419 & 1,106 & 290 \\
			\emph{Markor} &\tabincell{c}{Markdown \\Note Editor} & 2.0.1 &Dec. 2014 &50K$\sim$100K & 1.2K & 8,149 & 3,801 & 1,516 & 232 \\
			\emph{AnkiDroid} &\tabincell{c}{Advanced \\Flashcard Learning} & 2.9.6 &Jun. 2009 &5M$\sim$10M & 3K & 29,548 & 11,047 & 4,157 & 543 \\
			\emph{AnyMemo} &\tabincell{c}{Language \& \\Vocabulary Learning} & 10.11.4 &Jan. 2010 &100K$\sim$500K &122 &13,003 & 3,060 & 2,809 & 649 \\
			\emph{MyExpense} &\tabincell{c}{Personal \\Financial Assistant} & 3.0.9.1 &Mar. 2011 &500K$\sim$1M &278 &34,549 & 13,466 & 5,935 & 836 
			\\
			\hline 
		\end{tabular}
	\end{adjustbox}
\end{table*}

\begin{table}[t]
	\footnotesize
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	%% increase table row spacing, adjust to taste
	\renewcommand{\arraystretch}{1}
	% if using array.sty, it might be a good idea to tweak the value of
	% \extrarowheight as needed to properly center the text within the cells
	
	\caption{App subjects. \emph{Version} is the latest release versions
		at the time of our study. \#L and \#Br represent the numbers of code lines and branches, respectively (K=1,000, M=1000,000).}
	\vspace{-0.5pc}
	\label{table:app_subjects}
	\centering
	%% Some packages, such as MDW tools, offer better commands for making tables
	%% than the plain LaTeX2e tabular which is used here.
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{|c||c|c|c|c|c|c|c|c|}
			\hline
			App Name &\tabincell{c}{Version} &\tabincell{c}{\#Google Play\\Installations} &\tabincell{c}{\#GitHub\\Stars} &\tabincell{c}{\#L} &\tabincell{c}{\#Br} \\
			\hline \hline
			\emph{ActivityDiary} & 1.4.0 & 1K$\sim$5K &56 &4,238 &1,169  \\
			\emph{Transistor} & 3.2.2 & 10K$\sim$50K & 254  &3,024 & 1,003 \\
			\emph{Tasks} & 6.6.5 &100K$\sim$500K &1.3K &31,757 & 8,386  \\
			\emph{UnitConverter} & 5.5.1 &1M$\sim$5M &144 &1,525 & 304  \\
			\emph{RadioDroid} & 0.79 &50K$\sim$100K &323 &8,085 & 2,397  \\
			\emph{SkyTube} & 2.97 &100K$\sim$500K &843 &8,469 & 2,531  \\
			\emph{SimpleTask} & 10.3.0 &10K$\sim$50K & 390 & 2,512 & 1,022  \\
			\emph{Fosdem} & 1.6.2 &10K$\sim$50K & 111 & 5,563 & 1,419  \\
			\emph{Markor} & 2.0.1 &50K$\sim$100K & 1.2K & 8,149 & 3,801  \\
			\emph{AnkiDroid} & 2.9.6 &5M$\sim$10M & 3K & 29,548 & 11,047  \\
			\emph{AnyMemo} & 10.11.4 &100K$\sim$500K &122 &13,003 & 3,060  \\
			\emph{MyExpense} & 3.0.9.1 &500K$\sim$1M &278 &34,549 & 13,466  
			\\
			\hline 
		\end{tabular}
	\end{adjustbox}
\end{table}


%\begin{table*}[t]
%	\footnotesize
%	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%	%% increase table row spacing, adjust to taste
%	\renewcommand{\arraystretch}{1}
%	% if using array.sty, it might be a good idea to tweak the value of
%	% \extrarowheight as needed to properly center the text within the cells
%	
%	\caption{Code coverage of seed tests and their mutant tests for the app subjects. Line, Branch, Method represent line, branch and method coverage, respectively. The numbers in the brackets represent the coverage improvement of mutants \wrt seeds in terms of line, branch and method coverage, respectively.}
%	\vspace*{-0.5pc}
%	\label{table:code_coverage}
%	\centering
%	%% Some packages, such as MDW tools, offer better commands for making tables
%	%% than the plain LaTeX2e tabular which is used here.
%	\begin{tabular}{|c||c|c|c|c|c|c|c|c|c|}
%		\hline
%		App Name &\tabincell{c}{Line (\%)\\(seeds)} &\tabincell{c}{Line (\%)\\(mutants)} & \tabincell{c}{Branch (\%)\\(seeds)} & \tabincell{c}{Branch (\%)\\ (mutants)} & \tabincell{c}{Method (\%)\\(seeds)}& \tabincell{c}{Method (\%)\\(mutants)}  \\
%		\hline \hline
%		\emph{ActivityDiary} &45.9 & 65.0 (+19.1) &33.8 &48.2 (+14.4) &51.7 &70.0 (+18.3)  \\
%		\emph{Transistor} &58.5 & 63.1 (+4.6) &39.1 &43.9 (+4.8) & 61.0 & 65.5 (+4.5)  \\
%		\emph{Tasks} &28.6 & 33.9 (+5.3) &16.8 &23.3 (+6.5) &36.4 &40.9 (+4.5)\\
%		\emph{UnitConverter} &56.9 &71.6 (+14.7) &32.5 &61.5 (+29) &63.3 &73.7 (+10.4)  \\
%		\emph{RadioDroid} &46.6 &53.2 (+6.6) &31.9 &40.0 (+8.1) &48.8 &55.2 (+6.4) \\
%		\emph{SkyTube} &44.7 &51.9 (+7.2) &30.5 &37.3 (+6.8)  &50.0 &55.9 (+5.9) \\
%		\emph{SimpleTask} &31.3 & 33.7 (+2.4) &15.3 &19.3 (+4.0) &31.0 &34.7 (+3.7) \\ 
%		\emph{Fosdem} &60.0 &62.0 (+2.0) &39.7 &44.4 (+4.7) &69.0 &70.3 (+1.3) \\ 
%		\emph{Markor} &49.7 &57.7 (+8.0) &34.6 &43.8 (+9.2) &54.4 &60.0 (+5.6)  \\ 
%		\emph{AnkiDroid} &32.7 & 42.1 (+9.4) &20.8 &28.0 (+7.2) &41.0 &51.4 (+10.4)  \\ 
%		\emph{AnyMemo} &49.3 &53.5 (+4.2) &32.1 &38.7 (+6.6) &55.6 &58.3 (+2.7) \\
%		\emph{MyExpense} &25.1 &29.3 (+3.5) &15.6 &19.2 (+3.6) &32.3 &36.6 (+4.3)  \\
%		\hline
%		\textbf{Average} &\textbf{44.1}  &\textbf{53.0 (+8.9)} &\textbf{28.6} &\textbf{38.6 (+10.0)} &\textbf{49.5} &\textbf{56.0 (+6.5)}  \\
%		\hline 
%	\end{tabular}
%\end{table*}



\vspace{1pt}
\noindent{\emph{\textbf{Type 1: User data/setting lost}}}. This bug type leads to user data or setting lost. Sometimes, this bug type can bring severe consequences.
%and critical user complaints. For example, \emph{Markor}, a markdown note editor, ever had a data loss issue. One user critically complains ``\emph{Markor just went from hero to zero, in my books, as a file I had been working on just disappeared, without a trace! [...] I don't feel like I can currently trust markor with anything important, like the file I was just working on.}''.
\tool uncovered a data loss issue in \emph{Markor}, a markdown note editor.
The original content of a note file will be silently overwritten if the user creates another note file with the same name. Fig.~\ref{fig:example_bugs}(a) and Fig.~\ref{fig:example_bugs}(b), respectively, show the main page where a user can creates two notes with same name and the latter note's content overwrites that of the former one. The developer quickly confirmed and fixed this critical bug, and annotated it as a ``\emph{good first issue}''.

%Issue \#620

%Fig.~\ref{fig:example_bugs}(l) shows the same main page where the user only revises the file name of \emph{Note 2} to \emph{Note 1}. The \emph{Note 2} silently disappears, and the content of \emph{Note 2} overwrites \emph{Note 1}. 

\vspace{1pt}
\noindent{\emph{\textbf{Type 2: Function cannot proceed}}}. This bug type means one specific app function that works well before suddenly cannot proceed anymore and loses effect.
\tool found such an issue in \emph{SkyTube}, a YouTube video player.
Originally, a user can arbitrarily pause and play any video at his/her will.
However, if the user opens the menu, selects an option that plays the video in a browser, and returns back, he/she cannot play the video anymore --- clicking the play button cannot load the video; the play button cannot change to a pause button as well. After we reported this issue, the developer quickly confirmed and fixed it with positive feedback ``\emph{Thanks for the excellent bug report, it was very helpful to fix the bug!}``. 

%Fig.~\ref{fig:example_bugs}(c) shows its video playing page, where a user can arbitrarily pause and play any video at his/her will.
%Fig.~\ref{fig:example_bugs}(d) shows the same page after the user opens the menu (the three dots on the top right corner), selects an option that plays the video in a browser, and returns back. At this time, however, the user cannot play the video anymore --- clicking the play button cannot load the video; the play button cannot change to a pause button as well. After we reported this issue, the developer quickly confirmed and fixed it with positive feedback ``\emph{Thanks for the excellent bug report, it was very helpful to fix the bug!}``. 

%(Issue \#570)


%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=1.0\textwidth]{pics/example_bugs.pdf}
%	\vspace*{-1.7pc}
%	\caption{Examples of different functional bug types. In each group, the page at top shows the correct behavior, while the page at bottom shows the erroneous behavior, and the red boxes indicate the clues of each issue. }
%	\label{fig:example_bugs}
%\end{figure*} 

\noindent{\emph{\textbf{Type 3: Unexpected wrong behavior}}}.
This bug type means the specific functionality shows wrong behavior \wrt its previous correct behavior, \eg, an incorrect GUI page was erroneously opened, a deleted GUI view was suddenly restored. \tool found such an issue in \emph{ActivityDiary}. Fig.~\ref{fig:example_bugs}(e) shows the history detail page of \emph{Officework}, which was correctly opened after the user (1) starts \emph{Officework} from the main page, and (2) clicks its statistics region. However, if the user does three additional actions between (1) and (2) --- rename \emph{Officework} to another arbitrary name (say \emph{Shopping}); start another activity (say \emph{Gardening}); and undo \emph{Gardening} (\ie, return back to \emph{Shopping}). \emph{ActivityDiary} will erroneously open the history page of \emph{Gardening} rather than that of \emph{Shopping} (show in Fig.~\ref{fig:example_bugs}(f)). 
%If at this time the user modifies the history data of \emph{Gardening}, it will break data consistency. 
The developer commented ``\emph{(This is) definitely a bug, but I have to dig deeper in the code to get an idea how could it go wrong}''.

%(Issue \#288)
\vspace{1pt}
\noindent{\emph{\textbf{Type 4: Inconsistent GUI states}}}.
This bug type means the GUI states are inconsistent for specific functionality, which counters users' intuition on app function.
\tool found such an issue in \emph{Transistor}, a radio program player.
In the normal scenario,
Fig.~\ref{fig:example_bugs}(g) shows the page where a radio program is playing, and meanwhile a green playing indicator is shown near the program name. When the user stops the program, this green indicator will disappear. However, if the user renames the program when it is playing, and then stops it. The playing button will correctly change to a pause button, but the green playing indicator keeps there and indicates the program is playing (see Fig.~\ref{fig:example_bugs}(h)). This issue confuses users' intuition on the play-stop function. In fact, at the same time, the new program name will get lost.  
The developer was quite annoyed by this issue and commented ``\emph{This [...] related to the way Transistor handles stations internally. The root (cause) is so deep in the app's architecture, [...], it needs to wait for the big Kotlin re-write. Without a rewrite this would end in a bunch of nasty hacks.}''. Finally, the developer re-wrote the architecture, and fixed this issue.

%(Issue \#236)

\vspace{1pt}
\noindent{\emph{\textbf{Type 5: Duplicated GUI views}}}.
This bug type means some GUI views are erroneously duplicated.
\tool found such an issue in \emph{Tasks}, a task manager \& reminder.
Fig.~\ref{fig:example_bugs}(i) shows its main page when \emph{Task 1} was successfully created with a tag \emph{Meeting}. However, when this task was additionally inserted with two attachments (\eg, two pictures). \emph{Task 1} will be erroneously associated with two duplicated \emph{Meeting} tags (see Fig.~\ref{fig:example_bugs}(j)).

% (Issue \#811)
\vspace{1pt}
\noindent{\emph{\textbf{Type 6: Disappeared GUI views}}}.
This bug type means some GUI views inadvertently disappear.
\tool found such an issue in \emph{Fosdem}, a conference schedule browser.
Fig.~\ref{fig:example_bugs}(k) shows the correct \emph{Bookmarks} page. However, if the user (1) opens the menu (the three dots on the top right corner), (2) does two consecutive selections on the option ``Search events'', and (3) presses back, the filter option on the tool bar inadvertently disappears (Fig.~\ref{fig:example_bugs}(l)). Only restarting the app or reopening the page can recover this option view.

%(Issue \#811) 
\vspace{1pt}
\noindent{\emph{\textbf{Type 7: Incorrect GUI display information}}}.
This bug type means some views are incorrectly displayed. 
For example, \tool found such an issue in \emph{RadioDroid}. Due to this issue, all page titles are displayed as ``Setting'' if the user changes an irrelevant setting option. This option only alters the location of navigation menus between the page bottom and the navigation drawer.

%(Issue \#581)
\vspace{1pt}
\noindent{\emph{\textbf{Type 8: Functional GUI design issues}}}.
This bug type is related to the issue of functional GUI design, which
could confuse users and disrupt user experience.
For example, \tool found such an issue in \emph{RadioDroid}. 
The issue manifests itself as the \emph{history} page fails to record some ever played radio programs. After the discussion with developers, we know that \emph{RadioDroid} maintains two types of history data, \ie, \emph{history} and \emph{track history}. The \emph{track history} only records those radio programs with track information. However, \emph{RadioDroid} has never clearly differed these two types of history data on its GUIs (use the word \emph{history} for both functional pages). Finally, developers confirmed this issue and reworked the GUI design to avoid user confusion.

%(Issue \#775)


\begin{figure}[t]
	\centering
	\includegraphics[width=0.4\textwidth]{pics/affected_versions_and_time.pdf}
	\vspace{-1.0pc}
	\caption{Statistics of 33 confirmed functional bugs: (1) \#months they have resided (x-axis, in logarithmic scale); (2) \#affected releases (y-axis), before they were uncovered.}
	\label{fig:bug_quality}
\end{figure} 

%\begin{table}
%	\begin{minipage}{0.45\linewidth}
%		\centering
%		\captionof{figure}{Statistics of 33 confirmed functional bugs: (1) \#months they have resided (x-axis, in logarithmic scale); (2) \#affected releases (y-axis), before they were uncovered.}
%		\includegraphics[width=65mm]{pics/affected_versions_and_time.pdf}
%		\label{fig:bug_quality}
%	\end{minipage}\hfill
%	\begin{minipage}{0.5\linewidth}
%		\footnotesize
%		\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
%		%% increase table row spacing, adjust to taste
%		\renewcommand{\arraystretch}{1}
%		% if using array.sty, it might be a good idea to tweak the value of
%		% \extrarowheight as needed to properly center the text within the cells
%		
%		\caption{Quality of mutant tests generated by \tool. 1-O. D. E. (1-Occurrence Distinct Error), T. P. (True Positive), Insert. Pos. (Insert Position).}
%		\vspace{-2mm}
%		\label{table:mutation_ability}
%		\centering
%		%% Some packages, such as MDW tools, offer better commands for making tables
%		%% than the plain LaTeX2e tabular which is used here.
%		\begin{adjustbox}{max width=\textwidth}
%			\begin{tabular}{|c||c|c|c|c|c|c|c|}
%				\hline
%				App Name &\tabincell{c}{\#1-O. D. E.\\Seeds (A)} &\tabincell{c}{\#T. P.\\Seeds (B)} & \tabincell{c}{B/A} & \tabincell{c}{T. P. Insert.\\ Pos.  (\%)}   \\
%				\hline \hline
%				\emph{ActivityDiary} &15 & 8 &53.3\% & 30.4\%   \\
%				\emph{Transistor} &13 & 5 &38.5\% & 73.3\%   \\
%				\emph{Tasks} &10 & 7 &70.0\% &45.7\% \\
%				\emph{UnitConverter} &8 &2 &25.0\% & 35.0\%   \\
%				\emph{RadioDroid} & 11 & 5 & 45.0\% & 63.9\%  \\
%				\emph{SkyTube} & 15 & 2 & 13.3\% & 23.0\%   \\
%				\emph{SimpleTask} & 7 & 1 & 14.3\% & 25.0\%  \\ 
%				\emph{Fosdem} &9 &1 &11.1\% &60.0\%  \\ 
%				\emph{Markor} &11 &4 &36.6\% &52.5\%   \\ 
%				\emph{AnkiDroid} &14 & 0 & N/A & N/A   \\ 
%				\emph{AnyMemo} &12 & 4 & 33.3\% & 48.7\%  \\
%				\emph{MyExpense} &15 &2 &13.3\% &18.6\%   \\ 
%				\hline
%				\textbf{Total} &140  &41 &- &-   \\
%				\hline 
%			\end{tabular}
%		\end{adjustbox}
%	\end{minipage}
%	\vspace{-8pt}
%\end{table}

%\vspace{2pt}
%\noindent{\emph{\textbf{Quality of mutant tests}}}. Table~\ref{table:mutation_ability} gives the detailed analysis on the quality of mutants from \tool. \emph{\#1-O. D. E. Seeds} and \emph{\#T. P. Seeds} denote the number of seed tests that can generate 1-occurrence distinct error mutants and true positive mutants, respectively. Thus, \emph{B/A} indicates how many seed tests (in percentage) can generate true positive mutants. We can see, on average, {29.3\% (41/140)} of seed tests can be successfully mutated to uncover real functional bugs.
%\emph{T. P. Insert. Pos.} denotes, among those seed tests that can generate true positive mutants, on average how many insertion positions (in percentage) inserted with independent event traces can successfully create true positive mutants. 
%We can see the success rate ranges from {18.6$\sim$73.3\%} on these app subjects.
%Thus, these results show \tool has reasonable mutation ability to create true positive mutants at both seed test and insertion position levels without any human-provided tests.
%
%We also observe \tool's bug detection ability could be further improved by feeding high-quality seed tests that cover more meaningful app functionalities.
%For example, \tool's random seed generation produces only one meaningful seed test for finding the issues in \emph{SimpleTask} and \emph{Fosdem}, respectively.
%In the future, \tool can integrate the tests from human users or other tools.


\subsection{RQ4: Bug Types and Assorted Samples}
\label{sec:bug_types}

The functional bugs found by \tool are diverse. 
According to the bug consequences, we categorize the {33} functional bugs into six main types, 
including (1) \underline{4} \emph{user data/setting lost} issues, 
(2) \underline{7} \emph{function-cannot-proceed} issues, 
(3) \underline{7} \emph{unexpected wrong behavior} issues, 
(4) \underline{6} \emph{inconsistent GUI states} issues,
(5) \underline{7} \emph{incorrect GUI display} issues,
and (6) \underline{2} \emph{GUI functional design} issues.
%Fig.~\ref{fig:functional_failures_distribution} shows the distribution of these bug types.
%We can see user data/setting loss, function cannot proceed, unexpected wrong behavior and inconsistent GUI states are the top four bug types with most number of found issues, which are also more severe than other types.
We illustrate each functional bug type in the following.
Due to space limit, we leave the bug details (with GUI screenshots) in 
Appendix~\ref{sec:bug_example} for reference.
%Considering these bugs were triggered via sequences of events, we encourage the readers to watch the video illustrations~\cite{tool_link}, which can help understand the issues below more intuitively.

%\begin{figure}[t]
%	\centering
%	\includegraphics[width=\textwidth]{pics/functional_failure_distribution.pdf}
%	\vspace*{-2.0pc}
%	\caption{Distribution of different types of functional bugs discovered by \tool.}
%	\label{fig:functional_failures_distribution}
%\end{figure} 

\vspace{1pt}
\noindent{\emph{\textbf{Type 1: User data/setting lost}}}. This bug type loses user data or settings. Sometimes, it can bring severe consequences.
%and critical user complaints. For example, \emph{Markor}, a markdown note editor, ever had a data loss issue. One user critically complains ``\emph{Markor just went from hero to zero, in my books, as a file I had been working on just disappeared, without a trace! [...] I don't feel like I can currently trust markor with anything important, like the file I was just working on.}''.
\tool uncovered a data loss issue in \emph{Markor}, a markdown note editor.
The original content of a note file will be silently overwritten without any warning
if the user creates another note file with the same name. This issue was quickly confirmed and fixed, and annotated as a ``\emph{good first issue}''.

%Issue \#620

%Fig.~\ref{fig:example_bugs}(l) shows the same main page where the user only revises the file name of \emph{Note 2} to \emph{Note 1}. The \emph{Note 2} silently disappears, and the content of \emph{Note 2} overwrites \emph{Note 1}. 

\vspace{1pt}
\noindent{\emph{\textbf{Type 2: Function cannot proceed}}}. This bug type means one specific app function that works well before suddenly cannot proceed anymore.
\tool found such an issue in \emph{SkyTube}, a YouTube video player.
Originally, a user can arbitrarily pause and play any video at his/her will.
However, if the user opens the menu, selects an option that plays the video in a browser, and returns back, he/she cannot play the video anymore --- clicking the play button cannot load the video; the play button cannot change to a pause button as well. This issue was quickly fixed it with positive feedback ``\emph{Thanks for the excellent bug report, it was very helpful to fix the bug!}``. 

%Fig.~\ref{fig:example_bugs}(c) shows its video playing page, where a user can arbitrarily pause and play any video at his/her will.
%Fig.~\ref{fig:example_bugs}(d) shows the same page after the user opens the menu (the three dots on the top right corner), selects an option that plays the video in a browser, and returns back. At this time, however, the user cannot play the video anymore --- clicking the play button cannot load the video; the play button cannot change to a pause button as well. After we reported this issue, the developer quickly confirmed and fixed it with positive feedback ``\emph{Thanks for the excellent bug report, it was very helpful to fix the bug!}``. 

%(Issue \#570)


%\begin{figure*}[t]
%	\centering
%	\includegraphics[width=1.0\textwidth]{pics/example_bugs.pdf}
%	\vspace*{-1.7pc}
%	\caption{Examples of different functional bug types. In each group, the page at top shows the correct behavior, while the page at bottom shows the erroneous behavior, and the red boxes indicate the clues of each issue. }
%	\label{fig:example_bugs}
%\end{figure*} 

\noindent{\emph{\textbf{Type 3: Unexpected wrong behavior}}}.
This bug type means the specific functionality shows wrong behavior \wrt its previous correct behavior, \eg, an incorrect GUI page was erroneously opened, a deleted GUI view was suddenly restored. \tool found such an issue in \emph{ActivityDiary}. 
In the normal function, a user can click an activity $A$'s statistic region 
to show its history detail page.
However, if he/she renames this activity $A$ to $B$, and then starts another irrelevant activity $C$ and immediately undo $C$ (\ie, return back to $B$), 
and at this time click the activity $B$ will erroneously open the history detail page of $C$.
The developer has not expected this issue and commented ``\emph{(This is) definitely a bug, but I have to dig deeper in the code to get an idea how could it go wrong}''.

%(Issue \#288)
\vspace{1pt}
\noindent{\emph{\textbf{Type 4: Inconsistent GUI states}}}.
This bug type means the GUI states are inconsistent for specific functionality.
\tool found such an issue in \emph{Transistor}, a radio program player.
Normally, when a radio program is playing, \emph{Transistor} shows a green playing indicator near the program name; when the program is paused, this green indicator will disappear. However, if the user renames the program when it is playing, and then pauses it. The playing button will correctly change to a pause button, but the green playing indicator keeps there and indicates the program is playing. 
This is obviously incorrect.
The developer was annoyed by this issue and commented ``\emph{This [...] related to the way Transistor handles stations internally. The root (cause) is so deep in the app's architecture, [...], it needs to wait for the big Kotlin re-write.}''. 
Finally, the developer re-wrote the architecture, and fixed this issue.

%(Issue \#236)

\vspace{1pt}
\noindent{\emph{\textbf{Type 5: Incorrect GUI display}}}.
This bug type means some GUI views are incorrectly duplicated, lost or displayed.
For example, \emph{Tasks}, a task manager \& reminder,
has an issue: when a to-do task is created with a tag ``\emph{Meeting}`` 
and \emph{two} attachments, this task will be displayed 
with two duplicated tags ``\emph{Meeting}``.
\emph{Fosdem}, a conference schedule browser, will lost its
``\emph{filter}`` option icon on the toolbar under specific 
interactions.
\emph{RadioDroid} will display all its page titles as 
``\emph{Setting}'' if the user changes an irrelevant setting option.

%(Issue \#581)
\vspace{1pt}
\noindent{\emph{\textbf{Type 6: Functional GUI design issues}}}.
We found 2 functional design issues according to Genie's bug reports.
These bugs confuse users when using the app.
For example, in \emph{RadioDroid}, an issue manifests itself as the \emph{history} page fails to record some ever played radio programs. After the discussion with developers, we find developers mess up with \emph{history} and \emph{track history}.
Finally, developers confirmed this issue and reworked the GUI design to avoid user confusion.

%know that \emph{RadioDroid} maintains two types of history data, \ie, \emph{history} and \emph{track history}. The \emph{track history} only records those radio programs with track information. However, \emph{RadioDroid} has never clearly differed these two types of history data on its GUIs (use the word \emph{history} for both functional pages). Finally, developers confirmed this issue and reworked the GUI design to avoid user confusion.

%(Issue \#775)


%\vspace{1pt}
%\noindent{\emph{\textbf{Dynamic app features}}}. Modern Android apps provide dynamic features to improve user experience, which may incur false positives. For example, Fig.~\ref{fig:example_fps} (e) shows \emph{ActivityDiary}'s main page. When the user touches any activity (\eg, \emph{Woodworking}) in the list, the orders of activities will be dynamically shuffled (see Fig.~\ref{fig:example_fps} (f)). \emph{SkyTube} allow users to scroll down the video list to dynamically refresh the content. 
%These features affect oracle checking and lead to a lot of FPs.

%\vspace{1pt}
%\noindent{\emph{\textbf{Time/Number sensitivity}}}. This is another major reason that incurs a lot of FPs. For example, \emph{SkyTube} (see Fig.~\ref{fig:example_fps} (g)) displays the time progress and streaming speed information when playing videos. \emph{Markor} (see Fig.~\ref{fig:example_fps} (h)) shows each file's creation time and some file names contain a time tag after creation. These information severely affects oracle checking if without any filtering.



Table~\ref{table:fp_analysis} gives the detailed FP analysis results. \emph{\#F. P. Mutants} denotes the total number of FP mutants (computed by \emph{\#1-O. D. E. Mutants (refined)} and \emph{\#T. P. Mutants} in Table~\ref{table:detailed_testing_statistics}). 
The remaining columns denote the occurrences of specific FP root causes, respectively.
Specifically, we identified three classes of FP root causes. 
One class of FP root causes is related to the generability and oracle precision of our core techniques, \ie, independent view property violation (\emph{\#Independent Property}) and oracle checking limitation (\emph{\#Oracle Checking}). Another class is related to the app itself, including dynamic app features (\emph{\#App Features}) and time/number sensitivity (\emph{\#Time Sensitivity}). The third class is related to \tool's implementation trade-offs when no human knowledge is available, including \emph{imprecise layout types inferring} (\emph{\#Layout Types}), \emph{state abstraction} (\emph{\#State Abstraction}), and \emph{approximate execution} (\emph{\#Approx. Execution}).
Note that one FP mutant may be caused by multiple FP root causes at the same time. Thus, the sum of these seven root causes' occurrences may be larger than the total number of FP mutants.
We explain and illustrate each specific FP root cause below.


\begin{table}[t]
	\footnotesize
	\newcommand{\tabincell}[2]{\begin{tabular}{@{}#1@{}}#2\end{tabular}}
	%% increase table row spacing, adjust to taste
	\renewcommand{\arraystretch}{1}
	% if using array.sty, it might be a good idea to tweak the value of
	% \extrarowheight as needed to properly center the text within the cells
	
	\caption{Detailed analysis results on false positives (FPs).}
	\label{table:fp_analysis}
	\vspace*{-0.5pc}
	\centering
	%% Some packages, such as MDW tools, offer better commands for making tables
	%% than the plain LaTeX2e tabular which is used here.
	\begin{adjustbox}{max width=\textwidth}
		\begin{tabular}{|c||c||c|c|c|c|c|c|c|c|}
			\hline
			App Name &\tabincell{c}{\#F. P.\\ Mutants} & \tabincell{c}{\#I} &\tabincell{c}{\#O}  & \tabincell{c}{\#L} & \tabincell{c}{\#S}  & \tabincell{c}{\#Other} \\
			\hline \hline
			\emph{ActivityDiary} &58 & 31 & 5  &5 &2 & 15  \\
			\emph{Transistor} &21 & 4 & 6  & 0 & 0 &11 \\
			\emph{Tasks} &30 & 5 & 12  &0 &0 &13 \\
			\emph{UnitConverter} &58 &50  &0  &6 &0 &2  \\
			\emph{RadioDroid} &53 &8  & 0  &10 &25 &10  \\
			\emph{SkyTube} &62 &16  &0  &15  &0 &31  \\
			\emph{SimpleTask} &22  & 2 &11  &1  &0 &8  \\ 
			\emph{Fosdem}&42  & 0 & 1  &22 &19 &0  \\ 
			\emph{Markor}  &47 &3  &7  &5  &28 &4  \\ 
			\emph{AnkiDroid} &22 &16 & 0   &0  &2 &3  \\ 
			\emph{AnyMemo} &71 &34 &0  &12  &15 &10  \\
			\emph{MyExpense} &40 &0 & 0 &0  &35 &5  \\ 
			\hline
			\textbf{Total} &526  &169  &42 &76  &126 &112 \\
			\hline 
		\end{tabular}
	\end{adjustbox}
\end{table}
